PW-MAD: Pixel-wise Supervision for Generalized Face Morphing Attack Detection

A face morphing attack image can be verified to multiple identities, making this attack a major vulnerability to processes based on identity verification, such as border checks. Various methods have been proposed to detect face morphing attacks, however, with low generalizability to unexpected post-morphing processes. A major post-morphing process is the print and scan operation performed in many countries when issuing a passport or identity document. In this work, we address this generalization problem by adapting a pixel-wise supervision approach where we train a network to classify each pixel of the image into an attack or not, rather than only having one label for the whole image. Our pixel-wise morphing attack detection (PW-MAD) solution proved to perform more accurately than a set of established baselines. More importantly, PW-MAD shows high generalizability in comparison to related works, when evaluated on unknown re-digitized attacks. Additionally to our PW-MAD approach, we create a new face morphing attack dataset with digital and re-digitized samples, namely the LMA-DRD dataset that is publicly available for research purposes upon request.

==> vul_table.tex <==

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Attack}} & \multicolumn{2}{c|}{at FMR=0.1\%}                                & \multicolumn{2}{c|}{at FMR=1\%}                                  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                        & \multicolumn{1}{c|}{MMPMR(\%)} & \multicolumn{1}{c|}{FMMPMR(\%)} & \multicolumn{1}{c|}{MMPMR(\%)} & \multicolumn{1}{c|}{FMMPMR(\%)} \\ \hline
D-M                                           & 34.83                          & 39.29                           & 65.17                          & 68.93                           \\ \hline
PS-M                                          & 37.14                          & 43.37                           & 60.00                          & 69.88                           \\ \hline
\end{tabular}
\caption{vuln}
\label{tab:vul}
\end{table}
